Error Feedback Approach for Quantization Noise Reduction of Distributed Graph Filters

This work introduces an error feedback approach for reducing quantization noise of distributed graph filters. It comes from error spectrum shaping techniques from state-space digital filters, and therefore establishes connections between quantized filtering processes over different domains. Quantization noise expression incorporating error feedback for finite impulse response (FIR) and autoregressive moving average (ARMA) graph filters are both derived with regard to time-invariant and time-varying graph topologies. Theoretical analysis is provided, and closed-form error weight coefficients are found. Numerical experiments demonstrate the effectiveness of the proposed method in noise reduction for the graph filters regardless of the deterministic and random graph topologies.

==> refs.tex <==
@ARTICLE{1,
  author={Isufi, Elvin and Gama, Fernando and Shuman, David I and Segarra, Santiago},
  journal={IEEE Trans. Signal Process.}, 
  title={Graph Filters for Signal Processing and Machine Learning on Graphs}, 
  year={2024},
  volume={},
  number={},
  pages={1-32},
  keywords={Filter banks;Low-pass filters;Information filters;Signal processing;Filtering theory;Convolution;Machine learning;Graph signal processing;graph machine learning;graph convolution;filter identification;graph filter banks and wavelets;graph neural networks;distributed processing;collaborative filtering;graph-based image processing;mesh processing;point clouds;topology identification;spectral clustering;matrix completion;graph Gaussian processes},
  doi={10.1109/TSP.2024.3349788}}

@article{2,
  title={The emerging field of signal processing on graphs: Extending high-dimensional data analysis to networks and other irregular domains},
  author={Shuman, David I and Narang, Sunil K and Frossard, Pascal and Ortega, Antonio and Vandergheynst, Pierre},
  journal={IEEE Signal Process. Mag.},
  volume={30},
  number={3},
  pages={83--98},
  year={2013},
  publisher={IEEE}
}

@ARTICLE{3,
  author={Ortega, Antonio and Frossard, Pascal and Kovačević, Jelena and Moura, José M. F. and Vandergheynst, Pierre},
  journal={Proc. IEEE.}, 
  title={Graph Signal Processing: Overview, Challenges, and Applications}, 
  year={2018},
  volume={106},
  number={5},
  pages={808-828},
  keywords={Signal processing;Laplace equations;Graph theory;Machine learning;Data models;Social network services;Sampling methods;Graphical models;Graph signal processing (GSP);network science and graphs;sampling;signal processing},
  doi={10.1109/JPROC.2018.2820126}}

@inproceedings{4,
  title={Finite-precision effects on graph filters},
  author={Chamon, Luiz FO and Ribeiro, Alejandro},
  booktitle={Proc. Glob. Conf. Signal Inf. Process. (GlobalSIP)},
  pages={603--607},
  year={2017}
}

@INPROCEEDINGS{5,
  author={Nobre, Isabela Cunha Maia and Frossard, Pascal},
  booktitle={Proc. IEEE Int. Conf. Acoust., Speech, Signal Process. (ICASSP)}, 
  title={Optimized Quantization in Distributed Graph Signal Processing}, 
  year={2019},
  volume={},
  number={},
  pages={5376-5380},
  keywords={Quantization (signal);Distributed processing;Signal processing algorithms;Eigenvalues and eigenfunctions;Task analysis;Symmetric matrices;Graph signal processing;quantization;distributed processing;wireless sensor networks},
  doi={10.1109/ICASSP.2019.8682784}}

@article{6,
  title={Learning of robust spectral graph dictionaries for distributed processing},
  author={Thanou, Dorina and Frossard, Pascal},
  journal={EURASIP J. Adv. Signal Process.},
  volume={2018},
  number={1},
  pages={67},
  year={2018},
  publisher={Springer}
}

@INPROCEEDINGS{7,
  author={Saad, Leila Ben and Isufi, Elvin and Beferull-Lozano, Baltasar},
  booktitle={Proc. Glob. Conf. Signal Inf. Process. (GlobalSIP)}, 
  title={Graph Filtering with Quantization over Random Time-varying Graphs}, 
  year={2019},
  volume={},
  number={},
  pages={1-5},
  keywords={Quantization (signal);Wireless sensor networks;Topology;Finite impulse response filters;Covariance matrices;Nickel;Graph filters;Wireless sensor networks;Quan-tization;random links;Time-varying graphs.},
  doi={10.1109/GlobalSIP45357.2019.8969270}}

@ARTICLE{8,
  author={Ben Saad, L. and Beferull-Lozano, B. and Isufi, Elvin},
  journal={IEEE Trans. Signal Process.}, 
  title={Quantization Analysis and Robust Design for Distributed Graph Filters}, 
  year={2022},
  volume={70},
  number={},
  pages={643-658},
  keywords={Quantization (signal);Finite impulse response filters;Wireless sensor networks;Laplace equations;Eigenvalues and eigenfunctions;Task analysis;Topology;Distributed graph filtering;graph signal processing;graph filters;quantization;time-varying graphs},
  doi={10.1109/TSP.2021.3139208}}


@ARTICLE{9,
  author={Spang, H. and Schultheiss, P.},
  journal={IRE Trans. Commun.}, 
  title={Reduction of Quantizing Noise by Use of Feedback}, 
  year={1962},
  volume={10},
  number={4},
  pages={373-380},
  keywords={Noise reduction;Feedback;Nonlinear filters;Laboratories;Signal processing;Telephony;Quantization;White noise;Noise shaping;Signal analysis},
  doi={10.1109/TCOM.1962.1088681}}

@ARTICLE{10,
  author={Vaidyanathan, P.},
  journal={IEEE Trans. Circuits Syst.}, 
  title={On error-spectrum shaping in state-space digital filters}, 
  year={1985},
  volume={32},
  number={1},
  pages={88-92},
  keywords={Digital filters;Noise shaping;Noise reduction;State feedback;Signal processing;White noise;Signal processing algorithms;Instruments;Digital signal processing},
  doi={10.1109/TCS.1985.1085587}}


@article{11,
  title={Noise reduction strategies for digital filters: Error spectrum shaping versus the optimal linear state-space formulation},
  author={Higgins, W and Munson, D},
  journal={IEEE Trans. Acoust. Speech, Signal Processing},
  volume={30},
  number={6},
  pages={963--973},
  year={1982},
  publisher={IEEE}
}

@ARTICLE{12,
  author={Hinamoto, T. and Ohnishi, H. and Wu-Sheng Lu},
  journal={IEEE Trans. Circuits Syst. I}, 
  title={Roundoff noise minimization of state-space digital filters using separate and joint error feedback/coordinate transformation optimization}, 
  year={2003},
  volume={50},
  number={1},
  pages={23-33},
  keywords={Digital filters;State feedback;Noise reduction;Constraint optimization;IIR filters;Minimization;Quantization;Circuit noise;Iterative methods},
  doi={10.1109/TCSI.2002.807512}}

@ARTICLE{13,
  author={Wu-Sheng Lu and Hinamoto, T.},
  journal={IEEE Trans. Signal Process.}, 
  title={Jointly optimized error-feedback and realization for roundoff noise minimization in state-space digital filters}, 
  year={2005},
  volume={53},
  number={6},
  pages={2135-2145},
  keywords={Digital filters;IIR filters;State feedback;Feedforward systems;Iterative algorithms;Matrix converters;Degradation;Optimization methods;Relaxation methods;Noise reduction;Error-feedback matrix;roundoff noise in digital filters;state-space transformation;unconstrained optimization},
  doi={10.1109/TSP.2005.847847}}

@article{14,
  title={Advances in distributed graph filtering},
  author={Coutino, Mario and Isufi, Elvin and Leus, Geert},
  journal={IEEE Trans. Signal Process.},
  volume={67},
  number={9},
  pages={2320--2333},
  year={2019},
  publisher={IEEE}
}

@article{15,
  title={Autoregressive moving average graph filtering},
  author={Isufi, Elvin and Loukas, Andreas and Simonetto, Andrea and Leus, Geert},
  journal={IEEE Trans. Signal Process.},
  volume={65},
  number={2},
  pages={274--288},
  year={2016},
  publisher={IEEE}
}

@ARTICLE{16,
  author={Isufi, Elvin and Loukas, Andreas and Simonetto, Andrea and Leus, Geert},
  journal={IEEE Trans. Signal Process.}, 
  title={Filtering Random Graph Processes Over Random Time-Varying Graphs}, 
  year={2017},
  volume={65},
  number={16},
  pages={4406-4421},
  keywords={Finite impulse response filters;Topology;Laplace equations;Eigenvalues and eigenfunctions;Roads;Fourier transforms;Signal processing on graphs;graph filters;random graphs;random graph signals;graph signal denoising;graph sparsification},
  doi={10.1109/TSP.2017.2706186}}

@ARTICLE{17,
  author={Gao, Zhan and Isufi, Elvin and Ribeiro, Alejandro},
  journal={IEEE Trans. Signal Process.}, 
  title={Stochastic Graph Neural Networks}, 
  year={2021},
  volume={69},
  number={},
  pages={4428-4443},
  keywords={Stochastic processes;Graph neural networks;Convolution;Training;Topology;Network topology;Robot sensing systems;Graph neural networks;graph filters;distributed learning},
  doi={10.1109/TSP.2021.3092336}}

@article{18,
  title={GSPBOX: A toolbox for signal processing on graphs},
  author={Perraudin, Nathana{\"e}l and Paratte, Johan and Shuman, David and Martin, Lionel and Kalofolias, Vassilis and Vandergheynst, Pierre and Hammond, David K},
  journal={arXiv preprint arXiv:1408.5781},
  year={2014}
}sher={IEEE}
}

@ARTICLE{19,
  author={Gray, R.M. and Neuhoff, D.L.},
  journal={IEEE Trans. Inf. Theory}, 
  title={Quantization}, 
  year={1998},
  volume={44},
  number={6},
  pages={2325-2383},
  keywords={Quantization;Pulse modulation;History;Analog-digital conversion;Rate distortion theory;Gaussian noise;Gaussian processes;Data compression;Source coding},
  doi={10.1109/18.720541}}

@ARTICLE{20,
  author={Gray, R.M. and Stockham, T.G.},
  journal={IEEE Trans. Inf. Theory}, 
  title={Dithered quantizers}, 
  year={1993},
  volume={39},
  number={3},
  pages={805-812},
  keywords={Quantization;Random variables;Image reconstruction;Distortion;White noise;Fourier series;Sampling methods;Random processes;Information theory;Information systems},
  doi={10.1109/18.256489}}

@book{21,
  title={Funktionalanalysis},
  author={Werner, Dirk},
  year={2006},
  publisher={Springer-Verlag}
}
  


